Opening the Black Box: A Survey on the Mechanisms of Multi-Step Reasoning in Large Language Models

Large Language Models (LLMs) have demonstrated remarkable abilities to solve problems requiring multiple reasoning steps, yet the internal mechanisms enabling such capabilities remain elusive. Unlike existing surveys that primarily focus on engineering methods to enhance performance, this survey provides a comprehensive overview of the mechanisms underlying LLM multi-step reasoning. We organize the survey around a conceptual framework comprising seven interconnected research questions, from how LLMs execute implicit multi-hop reasoning within hidden activations to how verbalized explicit reasoning remodels the internal computation. Finally, we highlight five research directions for future mechanistic studies.

==> contents/future_directions.tex <==
\paragraph{Implicit Reasoning.}
Regarding the mechanistic study of implicit reasoning, several areas deserve further exploration.
First, research should move beyond simply finding correlations and use causal interventions to prove whether the identified internal representations are truly necessary for correct inference.
Second, many studies on the emergence of reasoning rely on toy models trained from scratch or indirect analyses of training data, which may not fully reflect how reasoning abilities develop in real-world LLMs. For example, while grokking has been proposed as a route to implicit multi-hop reasoning, most evidence comes from synthetic settings, leaving open how far it scales to harder, out-of-domain benchmarks and whether curricula or optimizer changes can make it computationally practical. Third, prior work suggests that what appears to be implicit multi-step reasoning often reflects shortcut exploitation (\textit{e.g.}, factual co-occurrence or surface cues), yet we still lack robust training-time interventions to reduce shortcut reliance—especially in large-scale, naturalistic pretraining where such shortcuts are ubiquitous and highly predictive. 
Finally, while many different mechanisms have been proposed, we still lack a unified framework to explain how these diverse findings fit together into a single theory of implicit reasoning.

\paragraph{Latent Reasoning.}
Beyond implicit and explicit Cot reasoning, an emerging direction is latent reasoning~\cite{DBLP:journals/corr/abs-2412-06769, DBLP:journals/corr/abs-2507-06203, DBLP:journals/corr/abs-2505-16782}, where multi-step reasoning is carried out in the model’s hidden states rather than discrete tokens. Compared to implicit reasoning—which denotes intermediate computations that emerge within a standard single forward pass of a fixed-depth transformer—latent reasoning typically introduces or exploits additional hidden-state computation (\textit{e.g.}, iterative refinement or recurrent state updates) while avoiding token-level reasoning traces. Relative to explicit CoT reasoning, latent reasoning may broaden the model’s effective expressive capacity while potentially reducing redundant token-level computation.
Although a growing body of work explores this paradigm, most studies focus on making it work in practice, and there is not yet a unified training framework or standard pipeline that reliably supports latent reasoning across tasks and models.
As a result, understanding how such hidden-space reasoning is represented and propagated remains an important direction for mechanistic research.


==> contents/introduction.tex <==
% \section{Introduction}
% Large language models (LLMs) have shown impressive abilities in solving complex reasoning tasks, including language understanding, mathematics, programming, and logical inference [CITES]. Central to these abilities is \textit{\textbf{multi-step reasoning}}, which involves drawing conclusions through a sequence of intermediate steps, where each step builds on the previous one. As one of the most fundamental forms of reasoning, it serves as the backbone of advanced tasks such as deep question answering, mathematical problem solving, logical deduction, code generation, and planning. 

% Background of Multi-Step Reasoning
Large Language Models (LLMs) have demonstrated an impressive ability to carry out \textit{\textbf{multi-step reasoning}}, which involves the process of drawing conclusions through a sequence of intermediate steps, where each step builds on the previous one. Multi-step reasoning has been widely regarded as one of the most fundamental forms of reasoning~\cite{hou_towards_mechanistic_multi_step,how_two_hop_in_context}. It serves as the backbone of advanced tasks such as deep question answering, mathematical problem solving, logical deduction, code generation, and planning~\cite{codex_model,wei2023chainofthought,gpt4_report,qwen25_report,llama3_herd_of_models,deepSeek_coder,deepSeek_R1}. 

% Forms of multi-step reasoning.
Multi-step reasoning in LLMs can take different forms. After extensive pretraining, models may exhibit an emergent ability of \textbf{\textit{implicit multi-step reasoning}}, \textit{i.e.}, producing the correct answer without explicitly verbalizing intermediate steps. For example, given the facts \textit{Peter was a mathematician}, \textit{mathematicians study logic}, and \textit{logic is central to computing}, one can infer that \textit{Peter contributed to the foundations of computing}. Although this conclusion requires a sequence of compositional inferences, an LLM can perform the reasoning entirely within its hidden activations, outputting only the final answer. 


In contrast to this latent process, LLMs can also engage in \textit{\textbf{explicit multi-step reasoning}}, where intermediate steps are verbalized rather than kept hidden. A widely used approach is \textit{chain-of-thought (CoT) prompting}~\cite{wei2023chainofthought,zeroshot-cot}, which instructs the model to ``think step-by-step'' and generate intermediate reasoning steps in natural language before arriving at the final answer. This simple technique has been shown to substantially improve performance on a wide range of reasoning tasks~\cite{Challenging_BIG_Bench,cot_survey_24,miner2025scheherazadeevaluatingchainofthoughtmath,to_cot_or_not,long_cot_survey}. 


% Following the success of CoT, recent \textit{long-thinking reasoning models}, such as OpenAI's O3~\cite{openai2025o3launch} and DeepSeek-R1~\cite{deepSeek_R1}, extend the depth and structure of CoT by combining inference-time scaling strategies~\cite{scaling_test_time_compute,inference_scaling_reward_modeling} with reinforcement learning~\citep[RL,][]{DPO_paper,let_verify_step_by_step}. Built on this, rapid progress has been made in leveraging such powerful multi-step reasoning capabilities of LLMs to build real-world applications, such as autonomous agents~\cite{survey_auto_agents}. 



% Rapid progress has been made in improving the multi-step reasoning capabilities of LLMs [CITE] and leveraging these capabilities to build real-world applications, such as autonomous agents. 

% Open research questions
However, despite such remarkable empirical success, we still only have a poor understanding of \textit{\textbf{the mechanisms underlying such multi-step reasoning capability}}. It is still unclear on \textit{how} LLMs internally carry out multi-step computations or \textit{why} training on next-token prediction over large text corpora gives rise to such reasoning abilities. Many fundamental questions remain open. For example, how do models decompose problems and carry information between steps internally? When a model answers correctly without showing work, is it truly reasoning or just recalling patterns? Why does explicit chain-of-thought often outperform implicit reasoning, and what does this reveal about internal representations? 
% For example, How do models decompose problems and carry information between steps internally? What did the model learn during training that allows it to reason? When a model answers correctly without showing work, is it truly reasoning or just recalling patterns? Why does explicit chain-of-thought often outperform implicit reasoning, and what does this reveal about internal representations? What principles govern the scaling of ``long-thinking'' models? These uncertainties highlight a gap between the impressive \textit{behavioral proficiency} of LLMs and our \textit{structural understanding} of that proficiency. 
% Bridging this gap is critical not only for interpreting model outputs, but also for designing methods that make reasoning more reliable, controllable, and robust. 
Bridging this gap is not only a matter of scientific curiosity of how reasoning emerges, but also a prerequisite for building reasoning systems that are more reliable, controllable, and aligned with human intentions. 
% Indeed, recent studies suggest that even when an LLM’s reasoning appears correct, it is unclear if the model followed the described reasoning or arrived at the answer via some shortcut or spurious correlation. Clarifying the inner workings of multi-step reasoning in LLMs is thus a pressing research area.

% A landscape of methods and questions.
Motivated by these goals, a growing literature seeks to open the black box of LLM multi-step reasoning. From the perspective of the \textit{\textbf{research problem}}, the interests distinguish between implicit and explicit reasoning. For implicit reasoning, work focuses on understanding how latent multi-hop computation is implemented~\cite{DBLP:conf/acl/BrinkmannSLSB24,how_two_hop_in_context}, how such ability is acquired during training~\cite{grokked_transformers,ye2025does}, and to what extent the reasoning relies on shortcuts~\cite{DBLP:conf/acl/YangKG0G25,DBLP:conf/acl/LinXYY25}. For explicit CoT reasoning, research examines where and when CoT improves performance~\cite{what_makes_cot_effective}, how it changes internal computation~\cite{think_doy_by_dot}, why it can outperform implicit reasoning~\cite{why_think_step_by_step}, how CoT capability itself is learned~\cite{xinyi_multi_path_aggregation}, and whether CoT explanations faithfully reflect internal processes~\cite{cot_is_not_explainability}. 
% In the emerging era of ``long-thinking'' models, new questions also arise about the principles governing deeper and more structured reasoning chains under inference-time scaling and RL~\cite{does_RL_really}.  

Beyond focusing on different research questions, existing studies also adopt different \textit{\textbf{analytical methods}}, which can be broadly divided into two categories. \textit{External diagnostic evaluations} treat the model as a black box and analyze its \emph{behavior} under controlled setting, \textit{e.g.}, when CoT helps, the learning dynamics of multi-step reasoning, and the scaling-law~\cite{to_cot_or_not,wang2025largerlanguagemodelsimply,topology_of_reasoning}. 
% how CoT answers differ from direct answers, and which prompt or task factors drive gains
Complementing this, \textit{internal mechanistic analyses} open the box to study how step-by-step reasoning is realized \textit{inside} the LLM, leveraging tools such as attention/head attribution, probing, and causal interventions to identify circuits, layerwise phases, and algorithmic patterns~\cite{grokked_transformers,mechanistic_cot,chen2025doeschainthoughtthink}. 


% \textit{internal mechanistic analyses} look \textit{inside} the model to uncover how step-by-step reasoning is realized, leveraging tools such as attention/head attribution, probing, and causal interventions to identify circuits, layerwise phases, and algorithmic patterns. 

% e.g., characterizing tasks where CoT helps or hurts performance【9】【16】, probing the learning dynamics of multi-step reasoning skills【22】, and measuring reasoning ability as model scale increases【22

% Our scope and contributions
In this paper, we aim to provide a comprehensive overview of research that seeks to \textit{uncover the mechanisms underlying LLM multi-step reasoning}. Although several surveys on LLM reasoning exist, they primarily focus on \textit{enhancing} reasoning --- through tool use, retrieval augmentation, or self-correction~\cite{reasoning_survey_huang,cot_24_survey,long_cot_survey} --- rather than on \textit{understanding} the mechanisms behind it. This survey aims to fill that gap. We systematically review progress on the mechanisms of multi-step reasoning, organizing the literature by the research problems posed, the analytical methods employed, and the key findings obtained. 

% Our goal is to present a clear picture of the current state of knowledge and to outline a coherent roadmap for future exploration in opening the black box of LLM reasoning. 

% We highlight emerging points of consensus, unresolved controversies, and methodological challenges, and we outline fruitful directions for future work. 

% There is still a lack of a survey from the perspective of understanding, providing a comprehensive view of the current understanding of multi-step reasoning: what research questions are being asked, what has been learned about how models reason, where consensus is beginning to emerge, where controversies remain, and what directions are most promising for further exploration. 

This survey is structured as follows. Section 2 provides a conceptual overview of the studies towards understanding LLM multi-step reasoning mechanisms. Section 3 focuses on implicit multi-step reasoning, examining how LLMs carry out latent multi-hop computations, how these abilities emerge during training, and to what extent the reasoning relies on shortcuts. Section 4 turns to explicit chain-of-thought reasoning, reviewing when and why explicit multi-step reasoning improves performance, what is known about the internal dynamics of CoT, and whether CoT enhances interpretability or risks an illusion of transparency. Finally, Section 5 outlines open problems and promising future directions. 


% This survey is structured as follows. Section 2 provides a \textit{conceptual overview} of the studies towards understanding LLM multi-step reasoning mechanisms. Section 3 focuses on \textit{implicit multi-step reasoning}, examining how LLMs carry out latent multi-hop computations, how these abilities emerge during training, and to what extent the reasoning relies on shortcuts. Section 4 turns to \textit{explicit chain-of-thought reasoning}, reviewing when and why explicit multi-step reasoning improves performance, what is known about the internal dynamics of CoT, how CoT capability is learned, and whether CoT enhances interpretability or instead risks an illusion of transparency. Section 5 discusses the unique mechanistic questions that arise in \textit{long-thinking CoT reasoning models}. Finally, Section 6 outlines open problems to be addressed and promising future directions towards gaining a deeper understanding of LLM reasoning. 

==> drafts/CoT_augments_computational_expressiveness.tex <==
\paragraph{CoT augments computational expressiveness.}
The most compelling explanation centers on \textit{computational complexity theory}, which reveals that CoT fundamentally expands the computational power of transformer architectures. 
% One explanation for the efficacy of CoT is that it enhances the computational expressiveness of the transformer architecture. 
% \citet{CoT_serial_problems} demonstrate that constant-depth transformers with finite precision can only solve problems in $\texttt{TC}^0$ without CoT, but with $T$ steps of CoT, these same transformers using constant-bit precision and $O(\log n)$ embedding size can solve any problem solvable by boolean circuits of size $T$. 
A series of theoretical works~\cite{DBLP:conf/nips/MerrillS23,DBLP:journals/tacl/MerrillS23,DBLP:conf/icml/0001CP23} have proved that transformer decoders without any intermediate steps can only solve problems that lie inside the fairly small circuit complexity class $\texttt{TC}^0$ and related logical classes. 
% Such models theoretically cannot solve inherently serial problems because the required computation depth grows with input size, while the model's depth is fixed~\cite{CoT_serial_problems,DBLP:conf/iclr/KimS25}. 
% CoT overcomes this inherent architectural limitation by enforcing a linear, recursive process. 
CoT overcomes this inherent architectural limitation by enabling the model to perform inherently serial computation, which effectively extends the model's computational depth. 
% which extends the theoretical depth of transformers. 
This allows the model to effectively simulate arbitrary recurrence, making inherently serial or recursive computations learnable where standard transformers cannot~\cite{CoT_serial_problems,DBLP:conf/iclr/KimS25}. 
% Each newly generated CoT token is appended to the context window and is subsequently attended to by the model during the generation of the following step. This self-attentive feedback loop effectively simulates arbitrary recurrence, making inherently serial or recursive computations learnable where standard transformers cannot~\cite{CoT_serial_problems,DBLP:conf/iclr/KimS25}. 
% enabling the model to perform inherently serial computations that standard transformers cannot~\cite{CoT_serial_problems}. 
% The theoretical power of this approach is significant.
% \citet{DBLP:conf/iclr/MerrillS24} proved that with a polynomial number of decoding steps, transformers with strict causal attention and projected pre-norm become equivalent to the complexity class $\texttt{P}$ (Polynomial Time). 
In theory, \citet{DBLP:conf/iclr/MerrillS24} proved that with a polynomial number of decoding steps, transformers with strict causal attention and projected pre-norm become equivalent to the complexity class $\texttt{P}$ (Polynomial Time). \citet{DBLP:conf/nips/FengZGY0W23} complemented the expressiveness theory with empirical evidence on mathematical and decision-making tasks. They showed that bounded-depth transformers cannot directly solve basic arithmetic or equation problems without an impractical increase in model size, while constant-size autoregressive transformers can effectively address these tasks by generating CoT derivations in a standard mathematical format. 

% All these results support the notion that Chain-of-Thought effectively increases the reasoning depth of LLMs, making inherently serial or recursive computations learnable where they otherwise were not.
% Theoretical work by \citet{CoT_serial_problems} shows that CoT strictly increases a transformer's expressiveness, enabling inherently serial computations that standard transformers cannot perform. With CoT, a model can simulate multi-step algorithms that a single forward pass cannot. This translates to markedly higher accuracy on tasks requiring multiple reasoning steps. 

==> drafts/CoT_explanability.tex <==
\paragraph{Evidence of CoT unfaithfulness.} 
% Recent studies discovered several evidence of this unfaithfulness. 
Recent studies reveal that CoT often functions as \textit{post-hoc rationalization} rather than a causal driver of its prediction~\cite{llm_dont_always_say,think_to_talk,cot_in_the_wild_not_faithful}. For example, \citet{llm_dont_always_say} demonstrated that when subtly reordering multiple-choice options in a question, the model's final choice often changed due to positional biases learned by the model. However, the model still tends to confabulate a logical-sounding CoT rationale that hides the actual spurious cause of its decision. 
% For instance, models influenced by input biases—such as the reordering of multiple-choice options—frequently generate coherent reasoning paths that justify the biased outcome while failing to mention the actual determining factor~\cite{Turpin2023}. 
Similarly, when correct answers are injected as hints, models invent spurious derivations to support the answer without acknowledging the hint's influence~\cite{dont_say_what_they_think-anthropic}. Furthermore, mechanistic analyses~\cite{cot_in_the_wild_not_faithful} found that models may make mistakes in their CoT and correct them internally, without the CoT reflecting the correction, known as ``silent error correction''. Another major evidence is called \textit{sycophancy}, where models tend to match user beliefs over truthful ones; even when models possess the correct internal knowledge, they frequently concede to incorrect user challenges or mimic user errors, generating plausible-sounding rationales to justify these compliant responses~\cite{understanding_sycophancy}. All the above evidence highlights a disconnect between the CoT rationale and the model's internal reasoning process or knowledge, challenging the view that CoT equates explanation. 



==> drafts/CoT_sample_complexity_robust.tex <==
We find that the success of CoT can be attributed to breaking down in-context learning of a compositional function into two distinct phases: focusing on and filtering data related to each step of the
composition and in-context learning the single-step composition function. Through both experimental and theoretical evidence, we demonstrate how CoT significantly reduces the sample complexity of in-context learning (ICL) and facilitates the learning of complex functions that non-CoT methods struggle with. 
\cite{DBLP:conf/nips/LiSGPO23}

Empirical and theoretical results confirm that many functions which stump a model under end-to-end prompting become learnable with CoT. For example, in a parity computation task (a classic “hard” boolean function), a transformer requires exponentially many training examples to succeed if it must infer parity in one step; but with CoT that same model can learn parity using a polynomial number of samples by solving it via stepwise XOR operations (Deng et al., 2023; Zhou et al., 2024)

Using a parity-learning setup, we demonstrate
that CoT can substantially improve sample efficiency even when the representation
power is sufficient. Specifically, with CoT, a transformer can learn the function
within polynomial samples, whereas without CoT, the required sample size is
exponential. \cite{DBLP:conf/iclr/WenZLZ25}

 One hypothesis about the inner workings of
CoT is that it breaks down originally complex tasks into smaller subtasks that
are more amenable to learning. We formalize this by showing possibility and
impossibility results of learning from in-context demonstrations with and without
CoT. In particular, with CoT, we examine a family of learning algorithms that
learn a task step-by-step, capable of composing simpler functions from individual
reasoning steps to form an overall complex function. This process reduces the
difficulty of learning a task to that of the hardest reasoning step in the chain.
Moreover, we prove Transformers can express this algorithm and thus they can
efficiently in-context learn arbitrary tasks as long as these tasks can be decomposed
into a finite number of subtasks, each of which are efficiently learnable.
\cite{DBLP:conf/iclr/Yang0W25}


In other words, CoT provides an inductive bias that matches the structure of complex multi-step problems, enabling the model to acquire skills that implicit reasoning struggles with. This aligns with the theoretical finding that CoT provably enables learning tasks that are otherwise unlearnable – the chain-of-thought essentially “unpacks” an intricate computation into a series of learnable transformations



==> drafts/When_and_where_CoT_help.tex <==
% and MMLU-Pro~\cite{MMLU_Pro}
\paragraph{On which tasks does CoT help?} To uncover this, \citet{to_cot_or_not} conduct a large-scale meta-analysis on 20 benchmarks and find that prompting with CoT yields large gains primarily on \textit{math and symbolic logic tasks}, with far smaller or even negative gains on other domains. For example, on knowledge-heavy benchmarks like MMLU~\cite{MMMU}, adding CoT steps barely changes accuracy unless the question involves a formal or arithmetic component. \citet{Challenging_BIG_Bench} similarly shows that many BIG-Bench Hard tasks~\cite{Big_Bench}, which had stumped standard few-shot prompts, become solvable with CoT. These were precisely tasks requiring multi-step reasoning, \textit{e.g.}, symbolic manipulation, compositional logic. 

\researchfinding{CoT prompting yields significant gains primarily in tasks involving \textit{mathematical, logical, or symbolic reasoning}. }


\researchfinding{In few-shot CoT prompting, models can still perform well with imperfect exemplar rationales, as long as the steps are coherent, relevant, and ordered, highlighting that CoT exemplars essentially teach \textit{how to think} (procedure), not what to think (facts).}

In zero-shot settings, \citet{zeroshot-cot} showed that simply appending ``Let’s think step by step'' to a question can elicit multi-step reasoning from models. Yet subsequent work shows that this effect is \textit{surprisingly sensitive to phrasing}. \citet{unzipping_black_box} systematically perturbed the trigger phrase and found that even minor wording changes can significantly alter performance. This suggests that zero-shot CoT operates less as a general instruction to reason and more as a \textit{trigger}, keyed to particular lexical patterns that models have implicitly learned to associate with reasoning behavior. 

\researchfinding{Zero-shot CoT is brittle to phrasing: even small rewordings of the ``Let’s think step by step'' cue can substantially affect whether the model engages in step-by-step reasoning.}


% \researchfinding{In few-shot prompting, CoT's benefit largely comes from imparting a structured reasoning format rather than from the factual correctness of exemplars. }

% \researchfinding{In few-shot CoT prompting, CoT's effectiveness stems less from the factual correctness of exemplars and more from their ability to provide a structured, stepwise reasoning format.}

==> drafts/implicit_reasoning.tex <==
% \subsection{Internal Mechanisms of Latent Multi-Hop Reasoning}

Multi-hop implicit reasoning is the process of answering a question by combining multiple pieces of information across several steps. Unlike explicit reasoning, the intermediate links are not directly stated and must be inferred using background knowledge or context. Mechanistic study of multi-hop implicit reasoning is important because it reveals whether models truly perform step-by-step reasoning or rely on shallow shortcuts. This understanding improves interpretability, trust, and guides the development of models that generalize more reliably.

\subsection{What are the internal mechanisms of latent multi-step reasoning?} 

Recent studies employing causal probing, mechanistic tracing, and representational analysis have advanced a nuanced understanding of this phenomenon, wherein intermediate results are computed internally but not explicitly produced. Despite methodological differences, these works collectively reveal a staged process in which mid-layer computations construct and transform intermediate representations that causally contribute to the final output.  

\textbf{Trees as a Structural Lens for Reasoning.}  An attention-based probing method, \textit{MechanisticProbe}, was introduced by \citet{hou2023mechanisticprobe} to recover reasoning trees from model internals. They further show that on synthetic and natural tasks with GPT-2 and LLaMA, LMs often perform procedural reasoning layer by layer, with lower layers selecting statements and higher layers executing reasoning steps. Complementing these findings, \citet{brinkmann2024mechanisticanalysis} analyze a small transformer trained on a symbolic tree pathfinding task, finding that it implements a backward chaining algorithm: deduction heads climb trees one level per layer, register tokens act as working memory for parallel subpaths, and a one-step lookahead heuristic compensates when chaining is insufficient. Together, these studies demonstrate that transformers can adopt structured, algorithm-like reasoning strategies beyond memorization, albeit within architectural depth limits.

\textbf{Layer Specialization.}  
Using \textit{Patchscopes} together with a novel intervention technique termed \textit{back-patching}, \citet{biran2024hopping} uncover a sequential computation pathway in which early layers identify the bridge entity, which is then propagated forward and exploited by later layers to complete the inference. Complementarily, \citet{li2024understanding}, through Logit Lens analysis and intervention experiments, show that implicit reasoning representations emerge in intermediate layers and exert a causal influence on the generation of final answers. Extending this perspective, \citet{yu2025back} investigate latent multi-hop reasoning in large language models (LLMs) via \textit{logit flow}, a neuron-level method for tracing how logits propagate across layers and positions. Their analysis reveals that single-hop predictions progress through four distinct stages---entity subject enrichment, entity attribute extraction, relation subject enrichment, and relation attribute extraction---each of which is localized to different layers.

\textbf{Why Latent Reasoning Fails at Times.} One of the most important aspects of the mechanistic analysis of LLMs is to understand why latent reasoning sometimes fails. \citet{biran2024hopping} discover that many such failures stem from delayed resolution of the first hop, and show that rerunning computations via back-patching can correct these errors, thereby exposing architectural limitations in transformer-based models. \citet{li2024understanding} find that failures frequently arise from the improper generation or utilization of implicit reasoning results. To address this issue, the authors propose \textsc{CREME}, a lightweight model-editing technique that patches specific multi-head self-attention (MHSA) modules, leading to improved compositional reasoning generalization with minimal disruption to unrelated predictions. In the context of two-hop queries (``$e_{1}$'s $r_{1}$'s $r_{2}$ is $e_{3}$''), \citet{yu2025back} show that errors often occur when high-layer features at the $r_{1}$ position overemphasize the intermediate entity $e_{2}$, outweighing the logits for the correct final entity $e_{3}$. This finding reveals that LLMs internally build and combine entity--relation representations in a staged manner, but positional interference can derail multi-hop reasoning. To mitigate this issue, they propose \textit{back attention}, which allows lower layers to access higher-layer states from other positions, thereby restoring crucial features and substantially improving multi-hop reasoning accuracy in both trained-from-scratch transformers and pretrained LLMs. \citet{yang2024large} use mechanistic probes—\textit{entity recall} and \textit{consistency} scores—to show that while LLaMA-2 reliably recalls bridge entities for the first hop, it only inconsistently applies them for the second. This breakdown highlights architectural limits that hinder reliable chaining of reasoning steps. 

\textbf{Distributional Reasoning.} Extending prior insights into multi-hop reasoning in LLMs, \citet{shalev2024distributional} introduce the concept of \textit{distributional reasoning}, wherein intermediate layers encode a probability distribution over multiple plausible intermediate answers. This representation gradually sharpens through a \textit{phase transition}—often mediated by feed-forward networks (FFNs)—which suppresses less likely candidates while amplifying the correct one, thereby transforming a diffuse distribution into a discrete final prediction.

 
Across these studies, a consistent computational picture emerges:  
\begin{enumerate}
    \item \textit{First-hop resolution} occurs in early-to-mid layers, often via attention heads that move source-entity information into positions associated with the bridge entity.  
    \item \textit{Intermediate representation construction}---either discrete or distributional---happens in mid layers, supported by attention and residual-stream storage.  
    \item \textit{Second-hop integration} is completed in mid-to-late layers, frequently mediated by FFNs that transform the intermediate representation into the final answer.  
    \item \textit{Causal dependency} is demonstrable: ablating or patching the relevant intermediate states significantly alters model outputs.  
\end{enumerate}

This convergence across causal, representational, and distributional analyses suggests that latent multi-hop reasoning in LLMs is not a monolithic capability but rather an orchestrated, layered process, with distinct modules and pathways specializing in different phases of the reasoning chain. Nevertheless, prior studies indicate that such implicit reasoning is constrained by the inherent architecture of transformers—for example, their fixed depth. To address these limitations, a growing body of work has proposed techniques aimed at enhancing performance.


% Example Research Question
% \researchquestion{1}{What are the internal mechanisms of latent multi-step reasoning?}

% Example Research Finding
% \researchfinding{CoT’s benefits are highly task-dependent and become most prominent in reasoning-intensive tasks.}

% 框框：Key Findings
% \result{Result V:}{Training with challenging irrelevant context leads to the strongest robustness and generalization across all pretraining settings.}

\subsection{How multi-step reasoning capability is acquired during training?}

Previous research \cite{olsson2022context, wei2022emergent} has observed an interesting phenomenon: modern deep learning models often undergo sudden shifts in their internal computational structure, accompanied by changes in input–output behavior. In particular, \citet{hooglandloss} shows that the training process of transformers can be divided into distinct stages, each marked by key transitions in both their internal organization and external performance. Similar to the earlier observation, the studies---\citet{wang2024grokked}, \citet{ye2025does}, and \citet{zhang2025complexity}---discovered a \textit{phase transition} in which training dynamics shift from early-stage \textit{memorization} to later-stage \textit{generalization} for multi-step reasoning tasks. This transition arises only after the model attains perfect in-distribution training accuracy and involves the gradual replacement or augmentation of memorization circuits with reasoning-oriented mechanisms. 

\textbf{Grokking}. Grokking \cite{power2022grokking} is a phenomenon in machine learning where a model initially appears to memorize training data without generalizing, but after much longer training (often far beyond achieving near-zero training error), it suddenly transitions to strong generalization performance. The phenomenon of transformers transitioning from early-stage \textit{memorization} to later-stage \textit{generalization} is investigated by \citet{wang2024grokked} through training transformers from scratch on symbolic reasoning tasks. They find that multi-hop reasoning emerges only through \textit{grokking}, where an early \textit{memorizing circuit} is gradually replaced by a more efficient \textit{generalizing circuit} due to optimization bias and weight decay. The speed of this replacement depends on the \textit{ratio of inferred to atomic facts} in training. Persistent OOD failures arise from limited \textit{cross-layer memory sharing}, where atomic facts not seen as second hops fail to reach higher layers, restricting compositional reuse. \citet{ye2025does} corroborate this phase transition, proposing a \textit{three-stage trajectory}: (i) rapid memorization, (ii) delayed in-distribution generalization, and (iii) slower cross-distribution generalization, with persistent OOD bottlenecks at the second hop. Mechanistically, they employ \textit{cross-query semantic patching} to localize the ``bridge'' entity and a \textit{cosine-based representational lens} to reveal that generalization coincides with \textit{mid-layer clustering} of intermediate entity representations. 

\textbf{Complexity Control}. \citet{zhang2025complexity} extend the picture by emphasizing the role of \textit{complexity control} in steering the phase transition. They show that smaller initialization scales and stronger weight decay bias the optimization process toward \textit{low-complexity, rule-like solutions} rather than high-complexity, memory-based mappings, thereby accelerating the emergence of reasoning capabilities. Using masking-based circuit probes and multiple complexity metrics (\textit{e.g.}, neuron condensation, embedding structure, stable rank), they demonstrate that such regularization not only improves OOD generalization but also alters the \textit{training pathway}, making the reasoning phase both more likely and more stable.  

In sum, all those works converge on the idea that multi-hop reasoning is \textit{acquired} through a phase transition from memorization to structured reasoning. \citet{wang2024grokked} highlight the \textit{data distribution} and \textit{circuit replacement dynamics}, \citet{ye2025does} focus on the \textit{representational organization} that accompanies generalization, and \citet{zhang2025complexity} identify \textit{optimization biases} that promote rule-based reasoning. Together, they suggest practical levers---adjusting the inferred-to-atomic ratio, encouraging cross-layer memory sharing, and applying stronger complexity control---to reliably induce reasoning acquisition during training.

\subsection{To what extent does the multi-step reasoning rely on shortcuts?}
\label{subsec:implicit:shortcuts}

 Previous studies \cite{elazar2023s, kang2023impact} have shown that LLMs's answer often rely on shortcuts. Following this line of work, \citet{yang2024large_shortcut, lin2025implicitreasoning, ju2024investigating, guo2025llms} conclude that large language models (LLMs) often achieve high apparent performance in multi-hop or multi-step tasks by \textit{exploiting shortcuts}---statistical or structural patterns in training data---rather than engaging in genuine compositional reasoning.

 \textbf{Factual Shortcuts}. \citet{ju2024investigating} investigates why LLMs often fail at multi-hop knowledge editing, showing that models rely on factual shortcuts—direct associations between the first and last entities—rather than true stepwise reasoning. Using Knowledge Neurons, a mechanistic interpretability tool, the authors trace which neurons encode these shortcuts and demonstrate that erasing them mitigates many editing failures. Similarly, \citet{yang2024large_shortcut} investigate whether LLMs solve multi-hop queries through genuine latent reasoning or by exploiting shortcuts such as subject–object co-occurrence and relation–object priors. Using Patchscopes, they show that successful latent reasoning aligns with the model constructing hidden-state representations of the bridge entity, whereas shortcut-prone cases bypass this internal process. Moreover, the authors introduce the shortcut-free \textbf{SOCRATES} dataset and demonstrate that measured \textit{latent composability}—the ability to answer multi-hop queries without explicitly generating the intermediate entity—drops by nearly a factor of three compared to shortcut-prone evaluations. 

 \textbf{Patter-based Shortcuts.} The study by Lin et al. [2025] on implicit multi-step arithmetic reasoning with GPT-2 shows that models can form step-by-step reasoning circuits when premises are fixed, verified via activation patching and attention tracing. But when premise order is randomized, performance collapses as models adopt a shortcut that treats all operations as commutative, failing especially with variable subtrahends. This suggests that models latch onto surface-structure regularities that work for many training examples but collapse when compositional structure deviates. \textit{How LLMs perform two-hop reasoning with distractors in context} is the central focus of \citet{guo2025llms}. They find that pretrained models default to a shortcut-like strategy of random guessing over all plausible answers. By reverse-engineering a minimal \textit{three-layer Transformer}, the authors uncover a sharp transition from this shortcut behavior to a structured \textit{sequential query mechanism}, where the model first retrieves the bridge entity and then the correct end entity. This mechanistic analysis shows how fine-tuning replaces shallow shortcut reliance with genuine multi-step reasoning circuits. 

 Taken together, these findings show that even when models succeed on multi-hop or multi-step reasoning benchmarks, much of that success can stem from \textit{heuristic or distributional shortcuts}---co-occurrence patterns in factual domains, or exploitable algebraic regularities in mathematical domains---rather than robust, generalizable reasoning mechanisms. This underscores the need for shortcut-free evaluation protocols (as in SOCRATES) and training setups that force models to construct and reuse intermediate representations even under adversarial input conditions.
